Learning-based lossless compression of 3D point cloud geometry

This paper presents a learning-based, lossless compression method for static point cloud geometry, based on context-adaptive arithmetic coding. Unlike most existing methods working in the octree domain, our encoder operates in a hybrid mode, mixing octree and voxel-based coding. We adaptively partition the point cloud into multi-resolution voxel blocks according to the point cloud structure, and use octree to signal the partitioning. On the one hand, octree representation can eliminate the sparsity in the point cloud. On the other hand, in the voxel domain, convolutions can be naturally expressed, and geometric information (i.e., planes, surfaces, etc.) is explicitly processed by a neural network. Our context model benefits from these properties and learns a probability distribution of the voxels using a deep convolutional neural network with masked filters, called VoxelDNN. Experiments show that our method outperforms the state-of-the-art MPEG G-PCC standard with average rate savings of 28% on a diverse set of point clouds from the Microsoft Voxelized Upper Bodies (MVUB) and MPEG. The implementation is available at https://github.com/Weafre/VoxelDNN.

==> AblationStudy.tex <==
%\par \textbf{Single-resolution encoder}: In order to show the effectiveness of the partitioning scheme, we perform the encoding experiments with fixed block size. Each $64 \times 64 \times 64$ block is divided into blocks of size 64, 32, 16 or 8 and a single bit is used to indicate the occupancy of each sub-block. In addition, occupied blocks will be encoded using VoxelDNN. Table \ref{table:singleres} shows the $bpov$ of each single-resolution encoder compared with multi-resolution VoxelDNN and G-PCC version 10. We observe that encoders with block size $32$ and $64$ outperform other single-resolution encoders with the gain over G-PCC more than $20\%$ on both MVUB and MPEG 8i. This can be explained by the fact that less contexts are provided to VoxelDNN at a lower resolution, and we thus do not have a good probability estimation. Besides, as we shown in the multi-res VoxelDNN, we should only partition sparse blocks into small blocks to eliminate the redundancy instead of dividing all blocks.
\input{table_bits_spent_on_block}
\begin{center}
\centering
\begin{table}[H]
\caption{Average bits percentage in total bitstream and number of occupied voxel for each block size with four partitioning levels }
\resizebox{\linewidth}{!}{ \begin{tabular}{M{1.7cm} P{3cm} P{3cm}}


Block size&\% in bitstream & Avg occupied voxels\\
\hline
64&71.5\%&7374\\

32&24.3\%&1224\\

16&4.0\%&119\\

8&0.2\%&13\\
\hline
\end{tabular}}
\label{table:bitpercentage}

\end{table}

\end{center}
\vspace{-1cm}
%Table \ref{table:bitpercentage} shows the bits percentage in the bitstream and the number of occupied voxel for each block size with four partitioning level encoder. It can be seen that most of the bits are spent for block 64 and 32, while block 16 and 8 only account for $4.2\%$ in bitstream. This explains why we only have a small gain when adding block 16 and 8 into the partitioner.

==> multires_vs_g-pcc.tex <==
\begin{center}
\centering
\begin{table}[H]
\caption{Average rate in bpov for the proposed VoxelDNN, compared with MPEG G-PCC and P(PNI).}
\resizebox{\linewidth}{!}{ \begin{tabular}{|M{1.7cm}|l|P{1.5cm}|P{2cm}|P{2.1cm}|P{2.3cm}|}
\hline
\multicolumn{2}{|c|}{\begin{bf} Test PC \end{bf}}  & \begin{bf} P(PNI)  \end{bf} & \begin{bf} G-PCC  \end{bf} & \multicolumn{2}{|c|}{\begin{bf} VoxelDNN \end{bf}}   \\
\hline
Dataset&Point Cloud & bpov&bpov&bpov&Gain over G-PCC\\
\hline
\multirow{5}{*}{MVUB}&Phil9 & 1.88 &1.23& 0.92&25.2\% \\
\cline{2-6}
%\hline
&Ricardo9 &1.79  &1.04& 0.72&30.7\% \\
\cline{2-6}
&Phil10 & - & 1.17& 0.83&29.0\% \\
\cline{2-6}
&Ricardo10 & - & 1.13& 0.75&29.9\% \\
\cline{2-6}
&\textbf{Average} &1.84 & \textbf{1.13}& \textbf{0.81}&\textbf{28.3\% }\\
\cline{2-6}

\hline
\multirow{5}{*}{MPEG 8i}&Loot10 & 1.69 &0.95&0.64 &32.6\% \\
\cline{2-6}
%\hline
&Redandblack10 &1.84  &1.09& 0.73&33.0\% \\
\cline{2-6}
&Boxer9 &-  &1.08& 0.76&29.6\% \\
\cline{2-6}
&Thaidancer9 &-&1.06 & 0.81 & 23.5\% \\
\cline{2-6}

&\textbf{Average} &\textbf{1.77} & \textbf{1.05}&\textbf{0.73 }&\textbf{30.4\% }\\
\hline



\hline
\end{tabular}}
\label{table:VoxelDNNresult}

\end{table}

\end{center}
\vspace{-1cm}

==> singleBlockResult.tex <==
\begin{center}
\centering
\begin{table*}[ht]
\caption{Average rate in bpov of single-resolution encoders, compared with MPEG G-PCC and multi-resolution VoxelDNN. }
\resizebox{\linewidth}{!}{ \begin{tabular}{|P{1.5cm}|l|P{1.5cm}|P{1.2cm}|P{1.5cm}|P{1.2cm}|P{1.5cm}|P{1.2cm}|P{1.5cm}|P{1.2cm}|P{1.5cm}|P{1.2cm}|P{1.5cm}|}
\hline
\multicolumn{2}{|c|}{\begin{bf} Test PC \end{bf}}  & \begin{bf} G-PCC  \end{bf} 
& \multicolumn{2}{|c|}{\begin{bf}  multi-res VoxelDNN \end{bf}}
& \multicolumn{2}{|c|}{\begin{bf} VoxelDNN - block 64 \end{bf}}
& \multicolumn{2}{|c|}{\begin{bf} VoxelDNN - block 32 \end{bf}}
& \multicolumn{2}{|c|}{\begin{bf} VoxelDNN - block 16 \end{bf}}
& \multicolumn{2}{|c|}{\begin{bf} VoxelDNN - block 8 \end{bf} } \\
\hline
Dataset&Point Cloud & bpov&bpov&Gain over G-PCC &bpov&Gain over G-PCC &bpov&Gain over G-PCC&bpov&Gain over G-PCC&bpov&Gain over G-PCC\\
\hline
\multirow{5}{*}{MVUB}&Phil9 & 1.23&  0.92&25.2\%&0.98 &20.3\% &0.97 &21.1\% &1.10 &10.5\% & 1.62&-31.7\%\\
\cline{2-13}
%\hline
&Ricardo9 &1.04 & 0.72&30.7\%& 0.79& 24.0\%&0.77 & 25.9\%& 0.90& 13.4\%&1.43&-37.5\% \\
\cline{2-13}
&Phil10 & 1.17 &  0.83&29.0\%& 0.89&23.9\% &0.88 & 24.7\%&1.02 & 12.8\% &1.51&-29.0\%\\
\cline{2-13}
&Ricardo10 & 1.13 &  0.75&29.9\%& 0.81&24.3\% &  0.80&25.2\% &0.94&12.1\% & 1.43&-33.6\% \\
\cline{2-13}
&\textbf{Average} &\textbf{1.13}  & \textbf{0.81}&\textbf{28.3\% } &\textbf{0.87}&\textbf{23.15\%} &\textbf{0.86 }&\textbf{24.3\%} &\textbf{0.99 }&\textbf{12.2\%}&\textbf{1.50}&\textbf{-33.0\%} \\
\cline{2-13}

\hline
\multirow{5}{*}{MPEG 8i}&Loot10 & 0.95 &0.64 &32.6\%&0.70 & 26.3\%&0.69 &27.3\% &0.87 & 8.4\% &1.49&-56.8\%\\
\cline{2-13}
%\hline
&Redandblack10 &1.09 & 0.73&33.0\% & 0.79&27.5\% &0.79 &27.5\% & 0.95&12.8\% & 1.57&-44.0\% \\
\cline{2-13}
&Boxer10 &1.08  & 0.76&29.6\%& 0.80&25.9\% &0.82 & 24.0\%&0.99 &8.3\% &1.61&-49.0\% \\
\cline{2-13}
&Thaidancer10 &1.06&  0.81 & 23.5\% &0.85 &19.8\% &0.86 &18.8\% & 1.03&2.8\% &1.59&-50\%\\
\cline{2-13}

&\textbf{Average} &\textbf{1.05} & \textbf{0.73 }&\textbf{30.4\% }&\textbf{0.79} &\textbf{24.9\%} &\textbf{0.79} &\textbf{24.5\% }&\textbf{0.96} &\textbf{8.1\% }&\textbf{1.57} &\textbf{-50.0\%}\\
\hline
\hline
\end{tabular}}
\label{table:singleres}

\end{table*}
\end{center}
\vspace{-1cm}





==> table_bits_spent_on_block.tex <==
\begin{center}
\centering
\begin{table}[H]
\caption{Average bits percentage for each block size in total bitstream}
\resizebox{\linewidth}{!}{ \begin{tabular}{M{1.7cm} P{4cm}}


Block size&\% in bitstream\\
\hline
64&71.5\%\\

32&24.3\%\\

16&4.0\%\\

8&0.2\%\\
\hline
\end{tabular}}
\label{table:bitpercentage}

\end{table}

\end{center}
\vspace{-1cm}
